SymBreak: Mitigating Quantum Degeneracy Issues in QLDPC Code Decoders by Breaking Symmetry

Quantum error correction (QEC) is critical for scalable and reliable quantum computing, but existing solutions, such as surface codes, incur significant qubit overhead. Quantum low-density parity check (qLDPC) codes have recently emerged as a promising alternative, requiring fewer qubits. However, the lack of efficient decoders remains a major barrier to their practical implementation. In this work, we introduce SymBreak, a novel decoder for qLDPC codes that adaptively modifies the decoding graph to improve the performance of state-of-the-art belief propagation (BP) decoders. Our key contribution is identifying quantum degeneracy as a root cause of the convergence issues often encountered in BP decoding of quantum LDPC codes. We propose a solution that mitigates this issue at the decoding graph level, achieving both fast and accurate decoding. Our results demonstrate that SymBreak outperforms BP and BP+OSD-a more complex variant of BP-with a $16.17\times$ reduction in logical error rate compared to BP and $3.23\times$ compared to BP+OSD across various qLDPC code families. With only an $18.97$% time overhead compared to BP, SymBreak provides significantly faster decoding times than BP+OSD, representing a major advancement in efficient and accurate decoding for qLDPC-based QEC architectures.

==> 04_formulation.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/Breaking.png}
    \caption{Breaking cycles in the Tanner graph to eliminate classical-like quantum trapping sets}
    \label{fig: breaking}
\end{figure*}

\section{Motivating Examples}
\label{sec:motivating example}

There are two types of quantum trapping sets (QTS) in the decoding process of quantum LDPC (qLDPC) codes using the belief propagation (BP) decoder. These QTSs can cause the decoder to fail to converge, preventing it from returning a correction that matches the error syndrome. Fortunately, we have identified that these QTSs arise from cycles in the Tanner graph. 
% By breaking these cycles, we can trade off some optimality in the correction operation for an increased success rate in returning a correction that properly resolves the syndrome. 

\subsection{Classical-like Quantum Trapping Set}
\cref{fig: CTS} provides an example of a classical (3,3) trapping set. As shown in \cref{fig: CTS}, this trapping set causes the BP decoder (Gallager A/B) to get stuck in the all-ones state, failing to converge to the correct all-zeros state. This issue arises due to a length-6 cycle in the Tanner graph. However, as illustrated in \cref{fig: breaking}, if we break this cycle by removing one of the even-degree stabilizers, the trapping set is eliminated, allowing the Gallager A/B decoder to correctly converge to the all-zeros state.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/TrappingSet.png}
    \caption{Classical-like (3, 3) quantum trapping set}
    \label{fig: CTS}
\end{figure}


\subsection{Degeneration-related Quantum Trapping Set}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/Blief_Split.png}
    \caption{Degeneration-related quantum trapping set}
    \label{fig: CTS}
\end{figure}
